VaPr: Variable-Precision Tensors to Accelerate Robot Motion Planning

High-dimensional motion generation requires numerical precision for smooth, collision-free solutions. Typically, double-precision or single-precision floating-point (FP) formats are utilized. Using these for big tensors imposes a strain on the memory bandwidth provided by the devices and alters the memory footprint, hence limiting their applicability to low-power edge devices needed for mobile robots. The uniform application of reduced precision can be advantageous but severely degrades solutions. Using decreased precision data types for important tensors, we propose to accelerate motion generation by removing memory bottlenecks. We propose variable-precision (VaPr) search optimization to determine the appropriate precision for large tensors from a vast search space of approximately 4 million unique combinations for FP data types across the tensors. To obtain the efficiency gains, we exploit existing platform support for an out-of-the-box GPU speedup and evaluate prospective precision converter units for GPU types that are not currently supported. Our experimental results on 800 planning problems for the Franka Panda robot on the MotionBenchmaker dataset across 8 environments show that a 4-bit FP format is sufficient for the largest set of tensors in the motion generation stack. With the software-only solution, VaPr achieves 6.3% and 6.3% speedups on average for a significant portion of motion generation over the SOTA solution (CuRobo) on Jetson Orin and RTX2080 Ti GPU, respectively, and 9.9%, 17.7% speedups with the FP converter.

==> tabs/bitwidth_combinations.tex <==
\renewcommand{\arraystretch}{1.2}

\begin{table}[t!]
\centering
\caption{FP data formats with different exponent and mantissa bits combinations.}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{|c|c|}
\hline
FP Data Format & Combinations                    \\ \hline \hline
FP4                     & E2M1                                     \\ \hline
FP5                     & E2M2, E3M1                               \\ \hline
FP6                     & E2M3, E3M2, E4M1                         \\ \hline
FP8                     & E2M5, E3M4, E4M3, E5M2, E6M1             \\ \hline
FP10                    & E2M7, E3M6, E4M5, E5M4, E6M3, E7M2, E8M1 \\ \hline
FP16                    & E5M10, E8M7                              \\ \hline
FP32                    & E8M23                                    \\ \hline
\end{tabular}
}

\label{tab:bitwidth_combinations}
\end{table}

==> tabs/combinatorial_search.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table}
\caption{Combinatorial search results for the six large tensors across 8 environments.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
                          & out\_spheres & grad\_out\_spheres & out\_vec   & closest\_pt & closest\_pt\_swept \\ \hline \hline
bookshelf\_small\_panda   & FP16 (E5M10) & FP4 (E2M1)         & FP5 (E2M2) & FP4 (E2M1)  & FP4 (E2M1)         \\ \hline
bookshelf\_tall\_panda    & FP16 (E5M10) & FP4 (E2M1)         & FP4 (E2M1) & FP4 (E2M1)  & FP4 (E2M1)         \\ \hline
bookshelf\_thin\_panda    & FP16 (E5M10) & FP5 (E2M2)         & FP5 (E2M2) & FP4 (E2M1)  & FP5 (E2M2)         \\ \hline
box\_panda                & FP16 (E5M10) & FP6 (E2M3)         & FP4 (E2M1) & FP5 (E3M1)  & FP6 (E3M2)         \\ \hline
box\_panda\_flipped       & FP16 (E5M10) & FP4 (E2M1)         & FP4 (E2M1) & FP5 (E3M1)  & FP4 (E2M1)         \\ \hline
cage\_panda               & FP16 (E5M10) & FP6 (E2M3)         & FP9 (E5M3) & FP7 (E4M2)  & FP4 (E2M1)         \\ \hline
table\_pick\_panda        & FP16 (E5M10) & FP6 (E2M3)         & FP6 (E3M2) & FP5 (E3M1)  & FP7 (E5M1)         \\ \hline
table\_under\_pick\_panda & FP16 (E5M10) & FP8 (E3M4)         & FP5 (E3M1) & FP6 (E4M1)  & FP7 (E5M1)         \\ \hline
\end{tabular}
}
\label{tab:combinatorial-search}


\end{table}

==> tabs/reduce_search_space.tex <==
% \renewcommand{\arraystretch}{1.2}
% \begin{table}
% \caption{Reduced search space filtered with per-tensor binary search results.}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|}
% \hline
%                                    & Original Search Space & Reduced Search Space & Reduction \\ \hline \hline
% bookshelf\_small\_panda   & 4084101                       & 583443                       & 7X             \\ \hline
% bookshelf\_tall\_panda    & 4084101                       & 583443                       & 7X             \\ \hline
% bookshelf\_thin\_panda    & 4084101                       & 583443                       & 7X              \\ \hline
% box\_panda                & 4084101                       & 583443                       & 7X             \\ \hline
% box\_panda\_flipped       & 4084101                       & 583443                       & 7X              \\ \hline
% cage\_panda               & 4084101                       & 583443                       & 7X             \\ \hline
% table\_pick\_panda        & 4084101                       & 555660                       & 7.35X              \\ \hline
% table\_under\_pick\_panda & 4084101                       & 555660                       & 7.35X             \\ \hline
% \end{tabular}
% }
% \label{tab:reduce-search}


% \end{table}


\renewcommand{\arraystretch}{1.2}
\begin{table}
\caption{Reduced search space filtered with per-tensor binary search results.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
Environment & Reduction & Environment & Reduction \\ \hline \hline
bookshelf\_small\_panda   & 7X 
& bookshelf\_tall\_panda & 7X \\ \hline

bookshelf\_thin\_panda    & 7X 
& box\_panda                & 7X             \\ \hline

box\_panda\_flipped       & 7X          
& cage\_panda               & 7X              \\ \hline

table\_pick\_panda        & 7.35X 
& table\_under\_pick\_panda & 7.35X             \\ \hline
\end{tabular}
}
\label{tab:reduce-search}


\end{table}

==> tabs/tensor_size.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table}
\caption{The average tensor size after VaPr search optimization.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|cll|rrrrrr|}
\hline
\multicolumn{3}{|l|}{\multirow{2}{*}{}}                                                                                                     & \multicolumn{6}{c|}{\textbf{Average Tensor Size (MB)}}                                                                                                                                                                                                                         \\ \cline{4-9} 
\multicolumn{3}{|l|}{}                                                                                                                      & \multicolumn{1}{l|}{\textbf{robot\_spheres}} & \multicolumn{1}{l|}{\textbf{grad\_out\_spheres}} & \multicolumn{1}{l|}{\textbf{sphere\_data}} & \multicolumn{1}{l|}{\textbf{closest\_pt}} & \multicolumn{1}{l|}{\textbf{out\_vec}} & \multicolumn{1}{l|}{\textbf{grad\_output}} \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{\textbf{small (125,2)}}}   & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{CuRobo}}}      & \textbf{IKO} & \multicolumn{1}{r|}{0.52}                    & \multicolumn{1}{r|}{0.35}                        & \multicolumn{1}{r|}{0.52}                  & \multicolumn{1}{r|}{0.52}                 & \multicolumn{1}{r|}{0.52}              & 0.10                                       \\ \cline{3-9} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{l|}{}                                      & \textbf{TO}  & \multicolumn{1}{r|}{0.66}                    & \multicolumn{1}{r|}{0.45}                        & \multicolumn{1}{r|}{5.58}                  & \multicolumn{1}{r|}{5.58}                 & \multicolumn{1}{r|}{0.66}              & 0.85                                       \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{VaPr-CuRobo}}} & \textbf{IKO} & \multicolumn{1}{r|}{0.25}                    & \multicolumn{1}{r|}{0.07}                        & \multicolumn{1}{r|}{0.26}                  & \multicolumn{1}{r|}{0.13}                 & \multicolumn{1}{r|}{0.10}              & 0.02                                       \\ \cline{3-9} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{l|}{}                                      & \textbf{TO}  & \multicolumn{1}{r|}{0.31}                    & \multicolumn{1}{r|}{0.09}                        & \multicolumn{1}{r|}{2.79}                  & \multicolumn{1}{r|}{1.37}                 & \multicolumn{1}{r|}{0.12}              & 0.22                                       \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{\textbf{medium (500,5)}}}  & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{CuRobo}}}      & \textbf{IKO} & \multicolumn{1}{r|}{2.07}                    & \multicolumn{1}{r|}{1.41}                        & \multicolumn{1}{r|}{2.07}                  & \multicolumn{1}{r|}{2.07}                 & \multicolumn{1}{r|}{2.07}              & 0.37                                       \\ \cline{3-9} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{l|}{}                                      & \textbf{TO}  & \multicolumn{1}{r|}{1.65}                    & \multicolumn{1}{r|}{1.14}                        & \multicolumn{1}{r|}{13.96}                 & \multicolumn{1}{r|}{13.96}                & \multicolumn{1}{r|}{1.65}              & 2.14                                       \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{VaPr-CuRobo}}} & \textbf{IKO} & \multicolumn{1}{r|}{0.99}                    & \multicolumn{1}{r|}{0.27}                        & \multicolumn{1}{r|}{1.04}                  & \multicolumn{1}{r|}{0.51}                 & \multicolumn{1}{r|}{0.38}              & 0.10                                       \\ \cline{3-9} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{l|}{}                                      & \textbf{TO}  & \multicolumn{1}{r|}{0.79}                    & \multicolumn{1}{r|}{0.22}                        & \multicolumn{1}{r|}{6.98}                  & \multicolumn{1}{r|}{3.44}                 & \multicolumn{1}{r|}{0.30}              & 0.55                                       \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{\textbf{large (2000,10)}}} & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{CuRobo}}}      & \textbf{IKO} & \multicolumn{1}{r|}{8.30}                    & \multicolumn{1}{r|}{5.63}                        & \multicolumn{1}{r|}{8.30}                  & \multicolumn{1}{r|}{8.30}                 & \multicolumn{1}{r|}{8.30}              & 1.45                                       \\ \cline{3-9} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{l|}{}                                      & \textbf{TO}  & \multicolumn{1}{r|}{3.32}                    & \multicolumn{1}{r|}{2.40}                        & \multicolumn{1}{r|}{27.93}                 & \multicolumn{1}{r|}{27.93}                & \multicolumn{1}{r|}{3.32}              & 4.30                                       \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{l|}{\multirow{2}{*}{\textbf{VaPr-CuRobo}}} & \textbf{IKO} & \multicolumn{1}{r|}{3.96}                    & \multicolumn{1}{r|}{1.08}                        & \multicolumn{1}{r|}{4.15}                  & \multicolumn{1}{r|}{2.04}                 & \multicolumn{1}{r|}{1.52}              & 0.37                                       \\ \cline{3-9} 
\multicolumn{1}{|c|}{}                                          & \multicolumn{1}{l|}{}                                      & \textbf{TO}  & \multicolumn{1}{r|}{1.58}                    & \multicolumn{1}{r|}{0.46}                        & \multicolumn{1}{r|}{13.96}                 & \multicolumn{1}{r|}{6.87}                 & \multicolumn{1}{r|}{0.61}              & 1.11                                       \\ \hline
\end{tabular}
}
\label{tab:tensor-size}


\end{table}

==> tex/evaluation.tex <==
\section{Evaluation}
\label{eval}
\subsection{Per-tensor Variable Precision Search}
\subsection{Cross-tensor Variable Precision Search}

==> tex/setup.tex <==
\section{Experimental Setup}
\label{setup}

